Improving Event Definition Following For Zero-Shot Event Detection

Existing approaches on zero-shot event detection usually train models on datasets annotated with known event types, and prompt them with unseen event definitions. These approaches yield sporadic successes, yet generally fall short of expectations. In this work, we aim to improve zero-shot event detection by training models to better follow event definitions. We hypothesize that a diverse set of event types and definitions are the key for models to learn to follow event definitions while existing event extraction datasets focus on annotating many high-quality examples for a few event types. To verify our hypothesis, we construct an automatically generated Diverse Event Definition (DivED) dataset and conduct comparative studies. Our experiments reveal that a large number of event types (200) and diverse event definitions can significantly boost event extraction performance; on the other hand, the performance does not scale with over ten examples per event type. Beyond scaling, we incorporate event ontology information and hard-negative samples during training, further boosting the performance. Based on these findings, we fine-tuned a LLaMA-2-7B model on our DivED dataset, yielding performance that surpasses SOTA large language models like GPT-3.5 across three open benchmarks on zero-shot event detection.

==> latex/introduction_old.tex <==
% Should change this to a teaser figure. Will look much better
\subfile{../tables/teaser_table}

% What's event extraction
Event extraction focusing on identifying key details of specific events in a given text, such as categorizing them based on a predefined event ontology and extracting associated arguments. This extracted information can be valuable for various applications, including constructing knowledge graphs~\cite{zhang2020aser}, generating text summaries~\cite{hsi2018event}, question answering~\cite{berant2014modeling,han2021ester} and identifying causal relationships~\cite{vo2020extracting,cui-etal-2022-event}. Beyond traditional NLP tasks, event extraction plays a crucial role in expert domains. In the fields of biology and medicine, it has been used to enhance downstream tasks by injecting additional knowledge~\citep{chandak2023building}. In the social sciences field, it aids in analyzing specific aspects~\citep{pan2021knowledge}. While event extraction models have been widely applied in multiple domains, they suffer from low generalizability towards unseen events due to the complexity of event structure.

Prior work has studied event extraction largely in a fully-supervised fashion~\cite{wadden2019entity,lin2020joint,nguyen2015event,nguyen2016joint,han2019deep,du2020event,huang2020biomedical,huang2020document,paolini2021structured}. While these work show promising performance on seen events, it cannot generalize well to long-tailed and unseen events ~\cite{ma2023star,zhang2022efficient}, which limit the availability of these EE models to an wider range of scenarios.\looseness=-1

Focusing on the low generalization issue, ~\citet{ma-etal-2023-dice} proposed to tackle event extraction in a low-resource scenario.
\citet{hsu-etal-2022-degree} propose to construct templates for events, which can utilize the good language understanding ability of pre-trained language models, and achieve good performance in low-resource setting, achieving data-efficient event extraction. 
Besides methods that reformat event extraction tasks, \citet{ma2023star} proposed to incorporate GPT models to generate pseudo data of unseen events, and further train the models to enable event-extraction ability on these events. While these data-efficient methods can enable models to do EE with a few data, they fall back on the flexibility to extract unseen events. With the need of training, these models cannot extract desired event information in real-time inference. Also for those expert domains, it can be difficult to acquire even a small amount of event examples for few-shot learning.\looseness=-1

Following the rapid improvement of Large Language Models (LLMs)~\citep{brown2020language, touvron2023llama, wang2023large, zhao2023mmicl} and instruction tuning (IT)~\citep{chung2022scaling, shao2022compositional}, \citet{wang2022code4struct, gao2023exploring, wei2023zero} propose to tackle event extraction by prompt-based inference-only method, which provides event definition as prompt to the instruction-tuned models and perform zero-shot event extraction directly.
% \citet{zhang2022efficient} do blablabla...
\citet{wang2022code4struct} leverages strong text-to-structure translation capability of LLMs to tackle structured prediction tasks.
\citet{gao2023exploring} conducts a series of experiments to explore the feasibility of ChatGPT\footnote{\hyperlink{https://chat.openai.com/chat}{https://chat.openai.com/chat}} for event extraction.
% (cite instruct-event) blablabla.
\citet{wei2023zero} transforms the zero-shot EE task into a multi-turn question-answering problem.
While these open the possibility to tackle EE with instruction-tuned models, the performance still suffers from the complexity of the events. Also, simply providing the event definition as instruction to the model, does not guarantee that  the model  "follows" the event definition~\citep{kung2023models,yin2023did}, leading to low performance.\looseness=-1

In this work, we aim to improve zero-shot event detection by training the model to better follow the event definition from a dataset characteristic perspective. Different from previous work focusing on the prompt strategies for LLMs, we further investigate the key charachatersitics of training data and event definition, to find the important factors for better event definition following.
Specifically, for the training data, we investigate the scaling law of the number of events, event definitions per events and samples per events. Also, we further look into the importance of incorporating event ontology information and hard negative samples during instruction tuning, to find an optimal recipe for training a zero-shot EE model.\looseness=-1

To conduct the experiments above, it's required to have a event extraction dataset, with large number of events, multiple event definition per events, and unify structure of the event definition, which is lack in all existing EE datasets.
We further propose Diverse Event Definition Dataset (DivED), which we utilize existing large language models to generate diverse event definition and samples, without the need of human annotator. DivED includes 3000+ events, each with 10 event definition and 10 samples. For each event definition, we specifically inject ontology information, including parents and sibling events. \looseness=-1

By experimenting on DivED dataset, we found that the key to improve model's event definition following is to incorporate large amount of events and diverse event definition. While a few training samples per events is also important to model's performance, using more does not scale up models performance on unseen events, meaning that training too much samples does not help model generalize to unseen event definition. We conclude that this is because the model relies on the generalizability to unseen event definition, and simply provide a few examples per event is enough for model to learn the event. Also, providing the event ontology information and negative examples is crucial for model's performance.\looseness=-1

Following the observation, we further train our model on the DivED dataset, and achieve State of the Art Zero-shot Event detection performance on ACE~\cite{doddington-etal-2004-automatic}, M2E2~\cite{li-etal-2020-cross} and PHEE~\cite{sun2022phee} test sets collected in TextEE~\cite{huang2023reevaluation}. By joint training with Geneva~\cite{parekh2023geneva} training set, we can further boost the performance, and surpass strong LLMs such as GPT-4 and Chat-GPT with less than 1/20 model parameters, showing the effectiveness and efficiency of our method. \looseness=-1
To conclude our main contributions are as follows:
\begin{enumerate}
  \item We systematically studied how different aspects of event extraction data impact large instruction-tuned models' event definition following and improve zero-shot event detection.\looseness=-1
  \item We designed a data generation pipeline to generate a Diverse Event Definition dataset (DivED) with 3000+ events and diverse event definitions. Our experiments on it reveal that diverse event and event definition is the key to improving zero-shot ED.\looseness=-1
  \item Our proposed model achieves SOTA results on ACE, M2E2, and PHEE datasets, surpassing OpenAI GPT models with less than 1/20 of the parameters. \looseness=-1
\end{enumerate}


% influence models performance and event definition following ability.

% , we investigate several key features to improve model's event definition following ability, including the importance of different charachteristic of the training data, the structure of the event definition. 

% investigate the key feature to improve zero-shot EE, by training the model to better follow instructions. Since the model relies on following the provided instructions during inference time to extract desired events, it is important for the model to learn to generalize to the unseen event definition.
% % (1) 

% In this work, we aim to improve zero-shot event extraction 

==> tables/inference_definition.tex <==
% \begin{table}[t]
% \centering
% \small
% % \scriptsize
% % \footnotesize
% \setlength{\tabcolsep}{0.3mm}
% \begin{NiceTabular}{l||ccc|ccc}
% \Hline
% \Block{1-1}{Metric $\rightarrow$\\Model $\downarrow$}
% &\Block{1-1}{\\Prec.} & \Block{1-1}{Trigger ID\\Rec.} & \Block{1-1}{\\F1}
% &\Block{1-1}{\\Prec.} & \Block{1-1}{Trigger CLS\\Rec.} & \Block{1-1}{\\F1}
% \\
% \Hline
% Ours & 
% 50.2 &
% 26.4 & 
% 34.7 &
% 41.1 &
% 24.5 &
% 30.7
% \\
% w/ DEG. ED & 
% 47.2 &
% 22.6 &
% 30.6 &
% 33.9 &
% 19.9 &
% 25.1
% \\
% \Hline
% Geneva &
% 54.8 &
% 16.3 &
% 25.2 &
% 20.5 &
% 15.1 &
% 17.4
% \\
% w/ DEG. ED & 
% 56.6 &
% 10.3 &
% 17.5 &
% 36.5 &
% 10.1 &
% 15.8
% \\

% % w/ DEGREE ED & \textcolor{red}{-1} & \textcolor{red}{-1} & \textcolor{red}{-1} & \textcolor{red}{-1} & \textcolor{red}{-1} & \textcolor{red}{-1} \\
% \Hline
% \end{NiceTabular}
% \caption{  We evaluate our trained models on the ACE dataset with event definitions from OneIE and DEGREE.
% }
% \label{table:inference-definition}
% \end{table}

\begin{table}[t]
\centering
\small
% \scriptsize
% \footnotesize
\setlength{\tabcolsep}{0.3mm}
\begin{NiceTabular}{l||ccc|ccc}
\Hline
\Block{1-1}{Metric $\rightarrow$\\Model $\downarrow$}
&\Block{1-1}{\\Prec.} & \Block{1-1}{Trigger ID\\Rec.} & \Block{1-1}{\\F1}
&\Block{1-1}{\\Prec.} & \Block{1-1}{Trigger CLS\\Rec.} & \Block{1-1}{\\F1}
\\
\Hline
Ours& 
46.7&
26.9&
34.2&
36.7&
24.1&
29.1
\\
w/ DEG. ED & 
42.57 &
22.90 &
29.79 &
31.67 &
20.23 &
24.69
\\
\Hline
Geneva &
47.7 &
14.5 &
22.2 &
18.2 &
13.8 &
15.7
\\
w/ DEG. ED & 
26.49 &
42.35 &
32.59 &
12.60 &
38.14 &
18.94
\\

% w/ DEGREE ED & \textcolor{red}{-1} & \textcolor{red}{-1} & \textcolor{red}{-1} & \textcolor{red}{-1} & \textcolor{red}{-1} & \textcolor{red}{-1} \\
\Hline
\end{NiceTabular}
\caption{  We evaluate our trained models on the ACE dataset with event definitions from OneIE and DEGREE.
}
\label{table:inference-definition}
\end{table}



==> tables/teaser_table.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{1mm}
\begin{NiceTabular}{p{0.73\linewidth}||p{0.2\linewidth}}
\Hline
\multicolumn{2}{c}{\textbf{Demonstration of Zero-shot EE}}\\
\hline
Input & Output \\
\hline
\textcolor{blue}{Sentence: The drug cartel funneled millions of dollars of illegal funds through a network of shell companies in different countries.} \textcolor{brown}{Event Type: Laundering}. \textcolor{green}{Event Definition: Money Laundering is the process of moving illicit funds through complex financial transactions, disguising the origin of the money and making them seem legitimate.} \textcolor{purple}{Parent Event: Fraud. Sons: Electoral Fraud, Laundering, Tunneling.} So what is the trigger? & The trigger is funneled. \\
\Hline
\Hline
\multicolumn{2}{c}{\textbf{Dataset Characteristic and Experiments}}\\
\hline
\textcolor{brown}{Event Type} & \# of Events \\
The name of the event type. & \\
\hline
\textcolor{green}{Event Definition(ED)} &\# of ED \\
The definition of the event type. &  per Event \\
\hline
\textcolor{blue}{Sample} & \# of Sample  \\
The positive training samples of an event. & per Event \\
\hline
\textcolor{purple}{Event Ontology} & \\
The ontology information. Including parent and sibling events. & Add/Remove \\
\hline
Hard Negative Samples & \\
Whether or not to use sibling events as Negative Samples during training & Add/Remove \\
\hline
% Active Instruction Tuning & &  \\
% \# of tasks in initial training set & 68 & 500 \\
% \# of task to select at $i$th iteration & 68 & $500*2^i$ \\
% \hline
% Evaluation & &  \\
% Evaluation Metrics & Rouge-L & \Block{2-1}{Human Eval\\GPT Eval} \\
% & & \\
\Hline
\end{NiceTabular}
% \vspace{-2em}
\caption{
% \footnotesize
Characteristics of event extraction data. During training, we will give the model \textit{Event Type}, \textit{Event Definition}, \textit{Event Ontology}, \textit{Example} and corresponding trigger to construct a positive samples, which has a ground truth trigger. We will further use unrelated events for the same sample to construct negative sample, which the ground truth trigger is None. For each different component, we conduct experiment to verify their impact to model's generalization performance to unseen events.\looseness=-1 
}
\vspace{-1em}
\label{table:exp-settings}
\end{table}
